Injecting linguistic knowledge into BERT for Dialogue State Tracking

Dialogue State Tracking (DST) models often employ intricate neural network architectures, necessitating substantial training data, and their inference process lacks transparency. This paper proposes a method that extracts linguistic knowledge via an unsupervised framework and subsequently utilizes this knowledge to augment BERT's performance and interpretability in DST tasks. The knowledge extraction procedure is computationally economical and does not require annotations or additional training data. The injection of the extracted knowledge can be achieved by the addition of simple neural modules. We employ the Convex Polytopic Model (CPM) as a feature extraction tool for DST tasks and illustrate that the acquired features correlate with syntactic and semantic patterns in the dialogues. This correlation facilitates a comprehensive understanding of the linguistic features influencing the DST model's decision-making process. We benchmark this framework on various DST tasks and observe a notable improvement in accuracy.

==> Assets/CPM_injection_layer_fig.tex <==
\begin{figure}[htp]
    \includegraphics[width=\linewidth]{Assets/layer.png}
    % \captionsetup{margin=3cm}
    \caption{$\Delta_{\text{baseline}}$ (difference to the baseline) of Joint Goal Accuracy (\%) of DST on WoZ and DSTC2 dataset with respect to the choice of BERT layer. A positive number indicates that observed performance exceeds baseline. $\Delta_{\text{baseline}} = 0$ is marked in red for clarity.}
    \label{fig:cpm_layer}
\end{figure}

==> Assets/CPM_radar.tex <==
\begin{figure}[thb]
    \centering
    \includegraphics[width=1.03\textwidth,height=\textheight,keepaspectratio]{Assets/radar_bw.png}
    \caption{Radar graphs of three groups (a, b, and c) of utterances with the same intent and slot tags, which are labelled in the group titles. The axes in the radar graph are the vertices of the polytope. The coordinate values
are the coefficients of the vertices of each utterance. }
    \label{fig:radars}
\end{figure}

==> Assets/fig_radars.tex <==
\begin{figure}[thb]
    \centering
    \includegraphics[width=1.03\textwidth,height=\textheight,keepaspectratio]{figs/radars_bw_l.png}
    \caption{Radar graphs of three groups (a, b, and c) of utterances with the same intent and slot tags, which are labelled in the group titles. The axes in the radar graph are the vertices of the polytope. The coordinate values
are the coefficients of the vertices of each utterance. }
    \label{fig:radars}
\end{figure}

==> Assets/hp.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|c|}
\hline
    & WoZ 2.0 & DSTC2 \\
    \hline
    \alpha & $2.68 \times 10^{-5}$ & $2.37 \times 10^{-5}$ \\
    \hline
    \beta & 8.38 & 7.56\\
    \hline
    \phi & 9.59 & 7.21 \\
    \hline
\end{tabular}
\caption{Best found hyperparameter values}
\label{hp}
\end{table}

==> Assets/multiwoz.tex <==
\begin{table*}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
    MultiWoZ version & v2.1 & v2.2 & v2.3 & v2.4 \\
     \hline
    train & 55.3 & 56.0 & 63.0 & 64.75 \\
    \hline
    dev & 54.65 & 55.47 & 63.47 & 66.16 \\ 
    \hline
    test & 55.3 & 56.0 & 63.0 & 64.75 \\
    \hline
\end{tabular}
    \caption{Joint Goal Accuracy (\%) of DST on 4 version of MultiWoZ datasets of the baseline model, and knowledge injected model. Results in bold are statically significant.}
    \label{cpm_result}
\end{table*}

==> Assets/slotupd.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|}
\hline
    Model & JGA \\
     \hline
    Baseline & 64.75 \\
    \hline
    CPM attention only & 63.70 \\
    \hline
    CPM coefficient only & 64.76 \\
    \hline
    Full CPM-assisted model & 66.16 \\
    \hline
\end{tabular}
    \caption{Ablation study result of CPM assisted model, measured by JGA (\%) 
 on MultiWoZ 2.4 dataset.}
    \label{cpm_ablate}
\end{table}
